The TESS-Keck Survey IV: A Retrograde, Polar Orbit for the Ultra-Low-Density, Hot Super-Neptune WASP-107b

We measured the Rossiter-McLaughlin effect of WASP-107b during a single transit with Keck/HIRES. We found the sky-projected inclination of WASP-107b's orbit, relative to its host star's rotation axis, to be $|\lambda| = {118}^{+38}_{-19}$ degrees. This confirms the misaligned/polar orbit that was previously suggested from spot-crossing events and adds WASP-107b to the growing population of hot Neptunes in polar orbits around cool stars. WASP-107b is also the fourth such planet to have a known distant planetary companion. We examined several dynamical pathways by which this companion could have induced such an obliquity in WASP-107b. We find that nodal precession and disk dispersal-driven tilting can both explain the current orbital geometry while Kozai-Lidov cycles are suppressed by general relativity. While each hypothesis requires a mutual inclination between the two planets, nodal precession requires a much larger angle which for WASP-107 is on the threshold of detectability with future Gaia astrometric data. As nodal precession has no stellar type dependence, but disk dispersal-driven tilting does, distinguishing between these two models is best done on the population level. Finding and characterizing more extrasolar systems like WASP-107 will additionally help distinguish whether the distribution of hot-Neptune obliquities is a dichotomy of aligned and polar orbits or if we are uniformly sampling obliquities during nodal precession cycles.

==> A Retrograde, Polar Orbit for WASP-107b/mcmc_results.tex <==
\begin{deluxetable}{lrrr}
\centering
\tablecaption{WASP-107b Rossiter--McLaughlin Parameters\label{tab:mcmcresults}}
\tablehead{
  \colhead{Parameter} & 
  \colhead{MCMC CI} & 
  \colhead{MAP value} &
  \colhead{Unit}
}
\startdata
\multicolumn{4}{l}{Model~Parameters} \\
$\sqrt{\vsini}\cos\lambda$ & $-0.309_{-0.154}^{+0.150}$     & -0.30  & \tablenotemark{a}  \\
$\sqrt{\vsini}\sin\lambda$ & $-0.126_{-0.771}^{+0.808}$     & -0.72  & \tablenotemark{a}  \\
$\cos i_s$                 & $-0.003_{-0.681}^{+0.682}$     & -0.56  &             \\
$\gamma$                   & $0.80_{-1.38}^{+1.36}$      & 0.97   &  m s$^{-1}$ \\
$\dot{\gamma}$             & $-20.83_{-10.94}^{+11.05}$  & -21.85 &  m s$^{-2}$ \\
$\sigma_{\text{jit}}$      & $2.61_{-0.51}^{+0.64}$      & 2.20   &  m s$^{-1}$ \\
$\log(|v_{cb}|)$           & $0.89_{-1.27}^{+1.18}$      & 2.17   & \tablenotemark{a}  \\
\hline
\multicolumn{4}{l}{Derived~Parameters} \\
% $\lambda$  & $196.419_{-85.060}^{+60.316}$  & -112.63  &  degrees     \\
$|\lambda|$& $118.1_{-19.1}^{+37.8}$        & 112.63   &  degrees     \\
$\vsini$   & $0.45_{-0.23}^{+0.72}$         & 0.61     &  km s$^{-1}$ \\
$v_{cb}$   & $-7.74_{-109.71}^{+7.33}$      & -149.41  &   m s$^{-1}$ \\
$i_\star$  & $28.17_{-20.04}^{+40.38}$      & 7.06     &  degrees     \\
$|\psi|$   & $109.81_{-13.64}^{+28.17}$     & 92.60    &  degrees     \\
\enddata
\tablenotetext{a}{
$\vsini$ is in km~s$^{-1}$ and $v_{cb}$ is in m~s$^{-1}$.
}
\end{deluxetable}

==> A Retrograde, Polar Orbit for WASP-107b/rvs.tex <==
\begin{deluxetable}{lccc}
\tablecaption{Radial Velocities of WASP-107\label{tab:rvs}}
\tablehead{
  \colhead{Time} & 
  \colhead{RV}   & 
  \colhead{$\sigma_{\rm{RV}}$} & 
  \colhead{Exposure time} \\
  \colhead{(BJD$_{\text{TDB}}$)} &
  \colhead{(m s$^{-1}$)} & 
  \colhead{(m s$^{-1}$)} & 
  \colhead{(s)}
}
\startdata
2458905.90111  &  5.05 & 1.50 & 900 \\
2458905.91189  &  6.43 & 1.42 & 883 \\
2458905.92247  &  0.14 & 1.49 & 862 \\
2458905.93288  & -1.35 & 1.65 & 844 \\
2458905.94266  & -0.25 & 1.45 & 783 \\
2458905.95204  & -5.28 & 1.44 & 745 \\
2458905.96141  & -2.40 & 1.37 & 797 \\
2458905.97098  & -3.40 & 1.46 & 754 \\
2458905.98004  &  2.45 & 1.37 & 727 \\
2458905.98927  & -5.52 & 1.45 & 780 \\
2458905.99888  &  2.07 & 1.48 & 792 \\
2458906.00848  &  4.21 & 1.37 & 776 \\
2458906.01796  & -0.58 & 1.38 & 775 \\
2458906.02768  &  0.83 & 1.47 & 817 \\
2458906.03780  &  3.07 & 1.49 & 836 \\
2458906.04780  & -3.01 & 1.26 & 818 \\
2458906.05771  &  0.02 & 1.45 & 796 \\
2458906.06752  & -3.72 & 1.49 & 795 \\
2458906.07703  &  3.61 & 1.33 & 773 \\
2458906.08654  &  1.27 & 1.38 & 790 \\
2458906.09648  & -2.88 & 1.45 & 837 \\
2458906.10657  & -5.39 & 1.44 & 818 \\
\enddata
\tablecomments{A machine readable version is available.}
\end{deluxetable}


==> A Retrograde, Polar Orbit for WASP-107b/systemprops.tex <==
\begin{deluxetable}{lrrr}
\centering
\tablecaption{Adopted parameters of the WASP-107 System\label{tab:systemprops}}
\tablehead{
  \colhead{Parameter} & 
  \colhead{Value} & 
  \colhead{Unit} &
  \colhead{Source} 
}
\startdata
$P_b$           & $5.7214742$                &  days    & 1    \\
$t_c$           & $7584.329897 \pm 0.000032 $& JD\tablenotemark{a} & 1    \\
$b$             & $0.07 \pm 0.07$            &          & 1    \\ 
$\iorbb$        & $89.887^{+0.074}_{-0.097}$& degrees  & 1    \\
$R_p/R_\star$   & $0.14434 \pm 0.00018$    &            & 1    \\
$a / R_\star$   & $18.164 \pm 0.037$       &           & 1    \\
$e_b$           & $0.06 \pm 0.04$          &            & 2  \\
$\omega_b$      & $40^{+40}_{-60}$         & degrees    & 2  \\
$M_b$           & $30.5 \pm 1.7$           & M$_\oplus$ & 2  \\
\hline
$P_c$          & $1088^{+15}_{-16}$        & days        & 2 \\
$e_c$          & $0.28\pm 0.07$            &             & 2 \\
$\omega_c$     & $-120^{+30}_{-20}$        & degrees     & 2 \\
$M_c\sin\iorbc$& $0.36 \pm 0.04$   & M$_J$       & 2 \\
\hline
$T_{\text{eff}}$ & $4245\pm 70$              & K         & 2 \\
$M_\ast$         & $0.683^{+0.017}_{-0.016}$ & M$_\odot$ & 2 \\
$R_\ast$         & $0.67\pm0.02$             & R$_\odot$ & 2 \\
$u_1$            & $0.6666 \pm 0.0062$       &           & 1 \\
$u_2$            & $0.0150 \pm 0.0110$       &           & 1 \\
\enddata
\tablenotetext{a}{Days since JD 2,450,000. Sources: (1) \citet{DaiWinn17}; (2) \citet{Piaulet2020}.}
\end{deluxetable}
